RMLStreamer-SISO: an RDF stream generator from streaming heterogeneous data

Stream-reasoning query languages such as CQELS and C-SPARQL enable query answering over RDF streams. Unfortunately, there currently is a lack of efficient RDF stream generators to feed RDF stream reasoners. State-of-the-art RDF stream generators are limited with regard to the velocity and volume of streaming data they can handle. To efficiently generate RDF streams in a scalable way, we extended the RMLStreamer to also generate RDF streams from dynamic heterogeneous data streams. This paper introduces a scalable solution that relies on a dynamic window approach to generate RDF streams with low latency and high throughput from multiple heterogeneous data streams. Our evaluation shows that our solution outperforms the state-of-the-art by achieving millisecond latency (compared to seconds that state-of-the-art solutions need), constant memory usage for all workloads, and sustainable throughput of around 70,000 records/s (compared to 10,000 records/s that state-of-the-art solutions take). This opens up the access to numerous data streams for integration with the semantic web.

==> _reviewing.tex <==
% Packages
\makeatletter
\def\uwave{\bgroup \markoverwith{\lower3.5\p@\hbox{\sixly \textcolor{red}{\char58}}}\ULon}
\font\sixly=lasy6 % does not re-load if already loaded, so no memory problem.
\makeatother

% Comments
%\newcommand{\todo}[1]{\noindent\textcolor{red}{{\bf \{TODO}: #1{\bf \}}}}
\newcommand{\TODO}[1]{\todo{#1}}
\newcommand{\citeneeded}{\textcolor{red}{{\bf [?!]}}}
\newenvironment{draft}{\color{gray}}{\color{black}}
\newenvironment{changed}{\color{black}}{\color{black}}

\usepackage{comment}
%Declare the boolean variable    
\newboolean{showremove} %Testblöcke anzeigen
%
%Set to OFF
\setboolean{showremove}{false}
\ifshowremove
  \newenvironment{toremove}{\color{red}}{\color{black}}
\else
  \excludecomment{toremove}
\fi


% Reviewers
\newcommand\ad[1]{{\color{green}\textbf{AD}: #1}}
\newcommand\bdm[1]{{\color{RoyalBlue}\textbf{BDM}: #1}}

% Changes
\newcommand\smo[1]{{\color{red}\textbf{SMO}: #1}}


% Annotations
\makeatletter
\font\uwavefont=lasyb10 scaled 700
\def\spelling{\bgroup\markoverwith{\lower3.5\p@\hbox{\uwavefont\textcolor{Red}{\char58}}}\ULon}
\def\grammar{\bgroup\markoverwith{\lower3.5\p@\hbox{\uwavefont\textcolor{LimeGreen}{\char58}}}\ULon}
\def\phrasing{\bgroup\markoverwith{\lower3.5\p@\hbox{\uwavefont\textcolor{blue}{\char58}}}\ULon}
\let\rephrase\phrasing
\newcommand\ins{\markoverwith{\textcolor{LimeGreen}{\rule[-0.5ex]{2pt}{0.4pt}}}\ULon}
\newcommand\remove{\bgroup\markoverwith{\textcolor{red}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon}
\makeatother

==> chapters/preliminaries.tex <==
\section{Preliminaries}

In this section, we discuss the concepts and terms regarding 
general stream processing and RDF generation which we will use throughout the rest of the paper. 
 
A \textit{data stream} is a flow of \textit{data records}. 
An RDF stream contains data records consisting of sets of 
triples (s,p,o) called an RDF graph, where s is the subject, 
p is the predicate, and o is the object. These RDF data records 
are tagged with the timestamp \textbf{t} which denotes their creation time. 

In order to compute aggregation of the data records, a state needs to 
be kept containing the most recent records in the data streams. 
This state is also known as \texit{windows}. The length of the windows
is denoted by its \texit{start-time} and end-time. All records whose 
timestamp value, $t  >= startTime$  and $t <= endTime$, are buffered 
inside the same window $w$ for processing. These windows could also 
be further partitioned according to some key value of the incoming 
records creating \textit{partitioned windows}. 
